Prize-collecting Network Design on Planar Graphs

In this paper, we reduce Prize-Collecting Steiner TSP (PCTSP), Prize-Collecting Stroll (PCS), Prize-Collecting Steiner Tree (PCST), Prize-Collecting Steiner Forest (PCSF) and more generally Submodular Prize-Collecting Steiner Forest (SPCSF) on planar graphs (and more generally bounded-genus graphs) to the same problems on graphs of bounded treewidth. More precisely, we show any $\alpha$-approximation algorithm for these problems on graphs of bounded treewidth gives an $(\alpha + \epsilon)$-approximation algorithm for these problems on planar graphs (and more generally bounded-genus graphs), for any constant $\epsilon > 0$. Since PCS, PCTSP, and PCST can be solved exactly on graphs of bounded treewidth using dynamic programming, we obtain PTASs for these problems on planar graphs and bounded-genus graphs. In contrast, we show PCSF is APX-hard to approximate on series-parallel graphs, which are planar graphs of treewidth at most 2. This result is interesting on its own because it gives the first provable hardness separation between prize-collecting and non-prize-collecting (regular) versions of the problems: regular Steiner Forest is known to be polynomially solvable on series-parallel graphs and admits a PTAS on graphs of bounded treewidth. An analogous hardness result can be shown for Euclidian PCSF. This ends the common belief that prize-collecting variants should not add any new hardness to the problems.

==> pcsf2.tex <==
\begin{tikzpicture}[y=-1cm]

% objects at depth 100:
\draw[black] (10.24889,31) -- (11,31);
\path (17.5,43.87556) node[text=black,anchor=base] {\large{}{\textbackslash}tex[][]\{\$w{\textasciicircum}1\_j\$\}};
\path (17.5,18.5) node[text=black,anchor=base] {\large{}{\textbackslash}tex[][]\{\$w\_1\$\}};
\draw[black] (20,39) -- (20.5,39) -- (20.5,43) -- (20.12444,43);
\draw[black] (20,42) -- (20.5,42);
\draw[black] (20,41) -- (20.5,41);
\draw[black] (20,40) -- (20.5,40);
\path (20.87333,39.74889) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$U\$\}};
\path (20.87333,40.62444) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$U\$\}};
\path (20.87333,41.62444) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$U\$\}};
\path (20.87333,42.74889) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$U\$\}};
\path (9,41.12444) node[text=black,anchor=base east] {\large{}{\textbackslash}tex[r][r]\{\$4U\$\}};
\draw[black] (9.5,43) -- (9.5,39) -- (10,39);
\path (9,49) node[text=black,anchor=base east] {\large{}{\textbackslash}tex[r][r]\{\$V\$\}};
\draw[black] (10,43) -- (9.5,43) -- (9.5,55) -- (10,55);
\path (18.24889,-3) node[text=black,anchor=base] {\large{}{\textbackslash}tex[][]\{\$2U\$\}};
\draw[black] (17.5,-4.5) -- (17.5,-4) -- (19,-4) -- (19,-4.5);
\path (9,1) node[text=black,anchor=base east] {\large{}{\textbackslash}tex[r][r]\{\$V\$\}};
\draw[black] (10,-5) -- (9.5,-5) -- (9.5,7) -- (10,7);
\path (14.5,-7.5) node[text=black,anchor=base] {\large{}{\textbackslash}tex[][]\{\$H\$\}};
\draw[black] (11.5,-6.5) -- (11.5,-7) -- (17.5,-7) -- (17.5,-6.5);
\filldraw[black] (11.5,6.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,6) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,5.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,4.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,4) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,3.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,3) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,2.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,2) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (19,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,1.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,1) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,0.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,0) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-0.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-0.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16.5,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15.5,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14.5,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13.5,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12.5,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-4.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-4.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-3.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-3.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-2.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-2.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-1.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,-1.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,10.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,10) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,9.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,9) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,8.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,8) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,7.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12.5,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13.5,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14.5,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15.5,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16.5,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,11) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,11.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,12) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,12.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,13) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,13.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (19,7) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,14) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,14.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,15) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,15.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,16) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,16.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,17) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,17.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,18) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,18.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,30.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,30) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,29.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,29) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,28.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,28) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,27.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,27) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,26.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,26) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (19,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,25.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,25) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,24.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,24) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,23.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,23) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16.5,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15.5,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14.5,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13.5,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12.5,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,19) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,19.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,20) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,20.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,21) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,21.5) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,22) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,22.5) ellipse (0.12444cm and 0.12444cm);
\path (17.5,38.5) node[text=black,anchor=base] {\large{}{\textbackslash}tex[][]\{\$w{\textasciicircum}2\_j\$\}};
\path (18,40.24889) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$c{\textasciicircum}2\_j\$\}};
\path (18,42.25111) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$c{\textasciicircum}1\_j\$\}};
\path (17.99778,41.24889) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$b\_j\$\}};
\path (19.49778,19.12444) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$a\_1\$\}};
\path (19.49778,7.12444) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$a\_2\$\}};
\path (19.49778,-4.87333) node[text=black,anchor=base west] {\large{}{\textbackslash}tex[l][l]\{\$a\_3\$\}};
\path (17.5,-5.37333) node[text=black,anchor=base] {\large{}{\textbackslash}tex[][]\{\$w\_3\$\}};
\path (17.5,6.5) node[text=black,anchor=base] {\large{}{\textbackslash}tex[][]\{\$w\_2\$\}};
\path (10,31.12222) node[text=black,anchor=base east] {\large{}{\textbackslash}tex[r][r]\{\$(0,0)\$\}};
\filldraw[black] (11.5,31.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,32.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,32.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,33.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,33.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,34.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,34.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,35.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,35.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,36.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,36.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,37.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,37.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,38.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16.5,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15.5,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14.5,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13.5,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12.5,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,42.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,42.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,41.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,41.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,40.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,40.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,39.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,39.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12.5,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13.5,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14.5,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15.5,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16.5,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,38.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,40.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,39.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,41.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,31.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,30.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,43.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,53.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,51.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,52.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16.5,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15.5,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14.5,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13.5,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12.5,51) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,51.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,51.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,52.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,52.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,53.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,53.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,54.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (12.5,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (13.5,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (14.5,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (15.5,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (16.5,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (17.5,54.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,50.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,50.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,49.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,49.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,48.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,48.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,47.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,47.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,46.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,46.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,45.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,45.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,44.99778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,44.49778) ellipse (0.12444cm and 0.12444cm);
\filldraw[black] (11.5,43.99778) ellipse (0.12444cm and 0.12444cm);

\end{tikzpicture}%

